Rewriting Ontological Queries into Small Nonrecursive Datalog Programs

We consider the setting of ontological database access, where an Abox is given in form of a relational database D and where a Boolean conjunctive query q has to be evaluated against D modulo a Tbox T formulated in DL-Lite or Linear Datalog+/-. It is well-known that (T,q) can be rewritten into an equivalent nonrecursive Datalog program P that can be directly evaluated over D. However, for Linear Datalog? or for DL-Lite versions that allow for role inclusion, the rewriting methods described so far result in a nonrecursive Datalog program P of size exponential in the joint size of T and q. This gives rise to the interesting question of whether such a rewriting necessarily needs to be of exponential size. In this paper we show that it is actually possible to translate (T,q) into a polynomially sized equivalent nonrecursive Datalog program P.

==> macros-local.tex <==
%%%%%%%%%% LOCAL MACROS %%%%%%%%%%

%\newcounter{banana}

%\newcommand{\impl}{\la}
%\newcommand{\limp}{\ra}


%%%%%%%%%% GENERAL

\newcommand{\lin}[2]{\mathsf{b}(#1,#2)}
\newcommand{\mgu}[2]{\textsf{MGU}(#1,#2)}
\newcommand{\f}[1]{\textsf{f}(#1)}
\newcommand{\ff}[1]{\textsf{ff}(#1)}
\newcommand{\fr}[2]{\textsf{fr}_{#1}(#2)}
\newcommand{\cover}[4]{#1 \prec_{#4}^{#3} #2}

\newcommand{\DB}{\mathit{DB}} \newcommand{\wrt}[0]{w.r.t.\ }


\newcommand{\ifdirection}{``$\Leftarrow$'' {}}
\newcommand{\onlyifdirection}{``$\Rightarrow$'' {}}

\renewcommand{\emptyset}{\varnothing}

\newcommand{\arc}{^\curvearrowright}

\newcommand{\qans}[3]{\mathsf{QAns}(#1,#2,#3)} % QAns(D,Sigma,q)

\newcommand{\relevent}[2]{\substack{#1,#2 \\ \twoheadrightarrow}} % QAns(D,Sigma,q)

%%%%%%%%%% DATABASES

\newcommand{\rel}[1]{\mathsf{#1}}
\newcommand{\attr}[1]{\mathit{#1}}
\newcommand{\const}[1]{\mathit{#1}}
\newcommand{\vett}[1]{\vec{#1}}

% extension of a relation
\newcommand{\ext}[2]{#1^{#2}}


%\newcommand{\tup}[1]{\langle #1 \rangle}

% Operator that returns the predicate to which a tuple belong
\newcommand{\pred}[1]{\mathit{pred}(#1)}

\newcommand{\atom}[1]{\underline{#1}}
\newcommand{\tuple}[1]{\mathbf{#1}}

\newcommand{\parent}[1]{\mathit{par}(#1)}
\newcommand{\dept}[1]{\mathit{depth}(#1)}

\newcommand{\mar}[1]{\hat{#1}}

%%%%%%%%%% DOMAINS

%\newcommand{\dom}{\Gamma} 
\newcommand{\freshdom}{\Gamma_N}
\newcommand{\variables}{\Gamma_V}
\newcommand{\adom}[1]{\mathit{dom}(#1)}
\newcommand{\var}[1]{\mathit{var}(#1)}
\newcommand{\varpos}[2]{\mathit{var}(#1,#2)}


%%%%%%%%%% CONCEPTUAL MODEL

\newcommand{\entities}{\mathit{Ent}}
\newcommand{\relationships}{\mathit{Rel}}
\newcommand{\attributes}{\mathit{Att}}
\newcommand{\symbols}{\mathit{Sym}}


%%%%%%%%%% DEPENDENCIES

\newcommand{\dep}{\Sigma}
\newcommand{\tdep}{\Sigma_T}
\newcommand{\edep}{\Sigma_E}
\newcommand{\fdep}{\Sigma_F}
\newcommand{\kdep}{\Sigma_K}
\newcommand{\ndep}{\Sigma_\bot}

\newcommand{\key}[1]{\mathit{key}(#1)}
\newcommand{\isa}[1]{\mathit{ISA}}


%%%%%%%%%% CONJUNCTIVE QUERIES

\newcommand{\Var}[1]{\mathit{Var}(#1)}
\newcommand{\head}[1]{\mathit{head}(#1)}
\newcommand{\body}[1]{\mathit{body}(#1)}
\newcommand{\arity}[1]{\mathit{arity}(#1)}
\newcommand{\conj}[1]{\mathit{conj}(#1)}

\newcommand{\ans}[3]{\mathit{ans}(#1,#2,#3)}


%%%%%%%%%% SETS OF VARIABLES

\newcommand{\ins}[1]{\mathbf{#1}}
\newcommand{\insA}{\ins{A}}
\newcommand{\insB}{\ins{B}}
\newcommand{\insC}{\ins{C}}
\newcommand{\insD}{\ins{D}}
\newcommand{\insX}{\ins{X}}
\newcommand{\insY}{\ins{Y}}
\newcommand{\insZ}{\ins{Z}}
\newcommand{\insK}{\ins{K}}
\newcommand{\insU}{\ins{U}}

%%%%%%%%%% CHASE STUFF

\newcommand{\chase}[2]{\mathit{chase}(#1,#2)}
\newcommand{\ochase}[2]{\mathit{Ochase}(#1,#2)}
\newcommand{\rchase}[2]{\mathit{Rchase}(#1,#2)}

% chase up to derivation depth #1:
\newcommand{\pchase}[3]{\mathit{chase}^{#1}(#2,#3)}
% chase up #1 application of the chase step:
\newcommand{\apchase}[3]{\mathit{chase}^{[#1]}(#2,#3)}
\newcommand{\aprchase}[3]{\mathit{Rchase}^{[#1]}(#2,#3)}
%
\newcommand{\level}[1]{\mathit{level}(#1)}
\newcommand{\freeze}[1]{\mathit{fr}(#1)}
\newcommand{\mods}[2]{\mathit{mods}(#1,#2)}
\newcommand{\subs}[2]{\gamma_{#1,#2}}


%%%%%%%%%% PARAGRAPH

\renewcommand{\paragraph}[1]{\textbf{#1}}
\newenvironment{proofsk}{\textsc{Proof (sketch).}}{$\Box$\newline}
\newenvironment{proofrsk}{\textsc{Proof (rough sketch).}}{$\Box$\newline}
\newenvironment{proofidea}{\textsc{Proof idea.}}{$\Box$\newline}


%%%%%%%%%% TGDS

\newcommand{\dg}[2]{\mathit{DG}(#1,#2)}
\newcommand{\rank}[1]{\mathit{rank}(#1)}

%%%%%%%%% Tick
\newcommand{\nc}{\newcommand}

\newcommand{\calC}{\ensuremath{{\cal C}}\xspace}
\newcommand{\bigO}{\ensuremath{{\cal O}}\xspace}

\newcommand{\dom}{\ensuremath{\text{dom}}\xspace}
\newcommand{\Neq}{\ensuremath{\text{Neq}}\xspace}
\newcommand{\Force}{\ensuremath{\text{Force}}\xspace}
\newcommand{\Num}{\ensuremath{\text{Num}}\xspace}
\newcommand{\DNum}{\ensuremath{\text{DNum}}\xspace}
\newcommand{\IfThen}{\ensuremath{\text{IfThen}}\xspace}
\newcommand{\IfTheni}{\ensuremath{\text{IfThen2}}\xspace}
\newcommand{\IfThenii}{\ensuremath{\text{IfThen3}}\xspace}

\newcommand{\rgoal}{\ensuremath{r_{\text{goal}}}\xspace} % Name of the
                                % final goal
\newcommand{\rtuples}{\ensuremath{r_{\text{tuples}}}\xspace} % Name of the
\newcommand{\rchaseok}{\ensuremath{r_{\text{chase}}}\xspace} % Name of the
\newcommand{\rquery}{\ensuremath{r_{\text{query}}}\xspace} % Name of the

\newcommand{\Ptuples}{\ensuremath{P_{\text{tuples}}}\xspace} % Name of the
\newcommand{\Pchase}{\ensuremath{P_{\text{chase}}}\xspace} % Name of the
\newcommand{\Pquery}{\ensuremath{P_{\text{query}}}\xspace} % Name of the

\newcommand{\serule}[3]{\ensuremath{ #2 \ra \exists #1\; #3}}  % tgd
                                % #1: existentially
                                % quantified variable, #2:
                                % body, #3: head

\newcommand{\srule}[2]{\ensuremath{ #1 \ra  #2}}  % tgd
                                % #1: body
                                % #2: head
\newcommand{\srulelb}[2]{\ensuremath{ #1 \ra\\\mbox{ }\hfill  #2\\}}  % tgd with linebreak
                                % #1: body
                                % #2: head

\newcommand{\drule}[2]{\ensuremath{ #2 :-  #1.}}  % Datalog rule
                                % #1: body
                                % #2: head
\newcommand{\longdrule}[2]{\begin{multline*} #2 :-\\
      #1.\end{multline*}}  % multi line Datalog rule
                                % #1: body
                                % #2: head

% Commands for commenting
% boxes with comments
\nc{\georg}[1]{\ \\ {\color{blue} \fbox{\parbox{\linewidth}{{\sc Georg}:\\  #1}}}}
\nc{\thomas}[1]{\ \\  {\color{blue} \fbox{\color{black}\parbox{\linewidth}{{\sc Thomas}:\\  #1}}}}


%corrections
\setul{}{0.3mm}
\setstcolor{red}
\newcommand{\oldnew}[3]{{\textcolor{blue}{\setlength{\fboxsep}{1pt}\fbox{\small #1}}} \st{#2} \textcolor{blue}{#3}}
% For submission change into
\renewcommand{\oldnew}[3]{#3}

% Changes by Georg [old text]{new text}
\nc{\gon}[2][]{\oldnew{G}{#1}{#2}} 
% Changes by Thomas[old text]{new text}
\nc{\ton}[2][]{\oldnew{T}{#1}{#2}}

\nc{\todo}[1]{\ \\ {\color{red} \fbox{\parbox{\linewidth}{{\sc ToDo}:\\  #1}}}}

\nc{\dlorfull}[2]{#1}
%\rnc{\dlorfull}[2]{#2}  % Uncomment this for full version

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

